Modularized Transfomer-based Ranking Framework

Recent innovations in Transformer-based ranking models have advanced the state-of-the-art in information retrieval. However, these Transformers are computationally expensive, and their opaque hidden states make it hard to understand the ranking process. In this work, we modularize the Transformer ranker into separate modules for text representation and interaction. We show how this design enables substantially faster ranking using offline pre-computed representations and light-weight online interactions. The modular design is also easier to interpret and sheds light on the ranking process in Transformer rankers.

==> old-version/sec-ablation.tex <==


% \subsection{Effects of Judger Block Layers}
% \label{subsec-block}
% \begin{table}[!ht]
% \caption{Ranking accuracy of \texttt{MORES} with varying number of judger blocks. The models were tested on the MS MARCO dataset with the Dev Queries.}
% \centering
% \begin{tabular}{ l || c }
% \hline \hline 
% Model & Dev Queries \\

%  & MRR@10 \\
%  \hline
% EARL ClsPool & \\
% \quad 1 block & 0.33015 \\
% \quad 2 blocks & 0.34422 \\
% \quad 3 blocks & 0.34255 \\
% \quad 4 blocks & 0.32732 \\
% \hline
% EARL ClsPool Tied & \\
% \quad 1 block & 0.33339\\
% \quad 2 blocks & 0.34561\\
% \quad 3 blocks & 0.34226\\
% \quad 4 blocks & 0.33071\\
%  \hline \hline 
% \end{tabular}
% \label{tab: n_jblocks}
% \end{table}
% The third experiment studies the effect of varying number of judger blocks in the relevance judging module. As described in section \ref{sec-method}, the judger block models the interaction between query and document. Within each block, a query to document attention captures query-document interactions, and a query side self-attention collects up the matching signals. Stacking up a total of N blocks means performing such operation for N times. In this section, we investigate how the number of iterations will affect the model's behaviors. 

% We take two variants of \texttt{MORES}, \texttt{MORES} ClsPool and \texttt{MORES} ClsPool Tied, and train variations with 1, 2, 3 and 4 judger blocks respectively and evaluate performance over the MS MARCO Dev queries. The results are summarized in table \ref{tab: n_jblocks}. We see for both model variants, one judger block is less effective compared to two, suggesting that a single round of interactions is not sufficient for matching. On the other hand, model performance saturates at two judger blocks, and further increasing the number to three does not improve performance. Increasing the number of blocks to four hurts the model's effectiveness. The decrease could be caused by our current way of initializing \texttt{MORES}. As we are not able to pre-train \texttt{MORES} from scratch due to hardware constraints, the judger blocks are initialized by borrowing parameters from a pre-trained BERT. These borrowed weights may not well align with the other parts of the \texttt{MORES} and can interrupt the hidden states, making the model starting point worse and the optimization problem harder.

\subsection{Impacts of Weight Initialization}
\begin{table}[!t]
\caption{Ranking Accuracy of \texttt{MORES} when using / not using attention weights copied from BERT to initialize Interaction Module. The models were tested on the MS MARCO dataset with the Dev Queries. }
\centering
\scalebox{0.85}{
\begin{tabular}{ l | c | c c c }
\hline 
 & Dev Queries & \multicolumn{3}{c}{TREC2019 DL} \\

 & MRR@10 & MRR & NDCG@10 & MAP \\
 \hline
MORES  & 0.3456 & 0.9283 & 0.7026 & 0.4777\\
- copy & 0.2723 & 0.843 & 0.6059 & 0.3702\\
% \hline
% EARL ClsPool Tied & \\
% \quad w/ copy & 0.3456 \\
% \quad w/o copy & 0.2414 \\
 \hline
\end{tabular}
}
\label{tab: weight-init}
\end{table}

%\zhuyun{Remind the readers what is our proposed weight initialization scheme}
Recall that in our proposed weight initialization scheme in \autoref{subsec: training-techniques},  BERT self-attention weight is copied to intialize IBs' cross attention, in order to avoid random initialization and to ease optimization. In this section, we take EARL models initialized with our proposed weight initialization scheme and compared them with ones that have cross attention weights initialized randomly. 
% We ablate two variants of \texttt{MORES}, \texttt{MORES} ClsPool and \texttt{MORES} ClsPool Tied, with randomly initialized judger block cross attention weight while holding other training setting the same as described in \ref{sec: implement-detail}. 
We evaluate the ablated models over the MS Marco Dev Queries and record results in \autoref{tab: weight-init}. Here, we see a drop in performance when cross attention weights are randomly initialized, indicating the importance of our proposed initialization method. 
% With such a deep transformer model, a set of uninitialized weights can largely increase optimization difficulty.





==> old-version/sec-exp-method.tex <==
\section{Experiments Methodology}
\label{sec: exp-method}
% This section discusses the experimental methodologies used in this work, including datasets, baselines and experimental methods, and implementation details.
This section discusses our supervised ranking and low-resource adaptation experiments. We also describe implementations of \texttt{MORES} and baseline.
\subsection{Supervised Ranking}
The supervised ranking experiment tests \texttt{MORES}'s ability to be trained and rank on the same corpus. We want to find out if \texttt{MORES} is as effective as SOTA ranker, on both single relevance and multiple relevance queries.

We use \textbf{MS MARCO passage ranking collection} (MS MARCO)~\cite{nguyen2016ms} and evaluate on two query sets with distinct characteristics:
\emph{Dev Queries} contains queries that have single relevant document with binary relevance labels. Following~\citet{nguyen2016ms}, we used MRR@10 to evaluate the ranking accuracy on this query set. \emph{TREC2019 DL Queries} is the evaluation set used in the TREC 2019 Deep Learning Track~\cite{craswell2019overview} and contains queries with multiple, graded relevance judgments.
Following~\citet{craswell2019overview}, we used MRR, NDCG@10, and MAP@1000 as evaluation metrics. All methods were evaluated in a \emph{reranking} task to re-rank the top 1000 documents of the MS MARCO official BM25 retrieval results.

\subsection{Adaptation to Low Resource Dataset}
We also test \texttt{MORES} with adaptation by in-domain fine-tuning model trained with MS MARCO on the target dataset. We first in-domain fine-tune all modules to verify that modular design does hurt transfer ability. Meanwhile, we seek to use adaptation to understand individual module. We use two experiments where only a subset of \texttt{MORES} modules are fine-tuned: only interaction module (adapt-interaction) or only representation modules (adapt-representation). The two study if adapting only interaction/representation is sufficient for adaptation to new domain. This effectively simulates a situation where we swap out modules from \texttt{MORES} to alter its function.

We use two new-domain low-resource datasets each with two query sets: \textbf{ClueWeb09-B} is a standard document retrieval collection with 50M web pages crawled in 2009.  Evaluation queries come from the TREC 2009-2012 Web Track. We used two variants of the queries: \emph{Title Queries} contains 200 short, keyword-style queries. \emph{Description Queries} contains 200 queries that are in the form of natural language statements or questions. \textbf{Robust04} is a news corpus with 0.5M documents. Evaluation queries come from TREC 2004 Robust Track, including 250 \emph{Title Queries} and 250 \emph{Description Queries}. We evaluate ranking performance with NDCG@20, MAP and Prec@20.
% \subsection{Datasets}
% We evaluate our model with three retrieval collections, each with two evaluation query sets.  

% \textbf{The MS MARCO passage ranking collection} (MS MARCO)~\cite{nguyen2016ms} is a passage retrieval collection with
% 8.8M passages. The
% training set contains approximately 0.5M pairs of queries and relevant passages. We used two evaluation query sets with distinct characteristics:
% \emph{Dev Queries} is the official development set from MS MARCO~\cite{nguyen2016ms}. It contains 6980 queries, where each query has one relevant document with binary relevance labels. Following~\cite{nguyen2016ms}, we used MRR@10 to evaluate the ranking accuracy on this query set.  \emph{TREC2019 DL Queries} is the  evaluation set used in the TREC 2019 Deep Learning Track shared retrieval task~\cite{craswell2019overview}. It contains 43 queries judged by NIST assessors with multiple, graded relevance judgments. Following~\cite{craswell2019overview}, we used MRR, NDCG@10, and MAP@1000 as the evaluation metric.
% All methods were evaluated in a \emph{reranking} task to re-rank the top 1000 documents of the MS MARCO official BM25 retrieval results~\cite{nogueira2019passage}.
 
% \textbf{ClueWeb09-B} is a standard document retrieval collection with 50M web pages crawled in 2009.  Evaluation queries come from the TREC 2009-2012 Web Track. We used two variants of the queries: \emph{Title Queries} contains 200 short, keyword-style queries. \emph{Description Queries} contains 200 queries that are in the form of natural language statements or questions. 

% \textbf{Robust04} is a news corpus with 0.5M documents. Evaluation queries come from TREC 2004 Robust Track, including 250 \emph{Title Queries} and 250 \emph{Description Queries}.

The experimental setup for ClueWeb09-B and Robust04 followed \citet{dai2019deeper}'s \emph{domain adaptation} setting, where we initially train the ranker on MARCO MS, and fine-tune and test it on the target dataset with 5-fold cross validation. All baselines and experimental rankers were used to re-rank the initial ranking provide by \citet{dai2019deeper}, which contains 100 candidate documents for each query. 
For handling long documents, all ranker follows the \citet{dai2019deeper}'s \texttt{BERT-FirstP} framework, which uses the title and the first passage to represent the document.  


\subsection{Baselines and Experimental Methods}
% We use two BERT-based neural rankers as baselines and compares them with different model variants of \texttt{MORES}.
We compare \texttt{MORES} with BERT ranker, the SOTA ranker fine-tuned from BERT, which process concatenated query document pair~\cite{Nogueira2019PassageRW, dai2019deeper}.  We use this baseline to demonstrate that the
%task dis-entanglement
\texttt{MORES} match SOTA performance.
%The second baseline is the \texttt{BERT-Siamese} ranker, a \emph{representation-based} ranker that encodes documents and queries each into a fixed-size embedding using BERT, with dot product as the similarity measure for ranking. In other words, it is a  neural ranker that is efficient, but loses token-level information for matching. We use it to show that the existence of token-level matching captured by cross-attentive operations in \texttt{MORES}'s relevance judging module is critical for matching performance. ~\cite{Reimers2019SentenceBERTSE} 
The baseline models inherit weights from the 12-layer BERT base model~\cite{Devlin2019BERTPO}. Following \citet{Nogueira2019PassageRW}, we fine-tune it to predict the relevance labels. %For the \texttt{BERT-Siamese} ranker, we follow \cite{Reimers2019SentenceBERTSE} and train ranker over hinge loss. We refer readers to those two papers for details. 
% The experimental methods include four \texttt{MORES} variants using different pooling and weight tieing. We studied two pooling functions for \texttt{MORES}'s relevance judging model (Eq.12): ClsPool and AvePool.  ClsPool takes the [CLS] token's representation to produce the final ranking score. AvePool takes the average of the token representations in the last layer. We also studied the use of weighting tying. The default \texttt{MORES} model uses separate weights for the query representation module and the document representation module. We test a tied variant that shares the query representation modules weight with the corresponding layers' weight in the document understanding module. 
% Combing the two pooling techniques and the use of weighting tieing gave us four \texttt{MORES} variants.

We test \texttt{MORES} with varied layers of Interaction Blocks (IB) to study effects of varying the complexity of query-document interaction. Models using 1 layer of IB~($1\times$ IB) up to 4 layers of IB ~($4\times$ IB) are included. 
% All \texttt{MORES} variants have Document Representation Module of 12 layers so that it can be initialized using BERT. 
% By default, the query understating module uses 10 transformer layers,  and the relevance judging module uses 2 layers of the judger blocks. Section~\ref{subsec-block} provides a study on the effects of the number of judger block layers.

We implemented baselines and \texttt{MORES} models using Pytorch \cite{pytorch} based on the huggingface  implementation of Transformers \cite{Wolf2019HuggingFacesTS}. Training details can be found in \autoref{sec:appendix-detail}.





==> old-version/sec-exp-results.tex <==
\section{Experiment Results}
\label{sec-experiments}
\begin{table*}[t]
\caption{Effectiveness of \texttt{MORES} models and baseline rankers on the MS MARCO Passage Corpus
}
\centering
\begin{tabular}{ l || c | c c c}
\hline \hline
 & \multicolumn{4}{c}{MS MARCO Passage Ranking}\\ 
\hline
 Models & Dev Queries & \multicolumn{3}{c}{ TREC2019 DL Queries}  \\ 
 
 & MRR & MRR & NDCG@10 & MAP \\  
 \hline
 BERT ranker  & 0.3527 & 0.9349 & 0.7032 & 0.4836  \\
% BERT-Siamese ranker & \zhuyun{} & \zhuyun{} & \zhuyun{} & \zhuyun{}\\
 \hline
 %MORES & \\
 MORES $1\times$ IB & 0.3334 & 0.8953	& 0.6721 & 0.4516 \\
 MORES $2\times$ IB & 0.3456 & 0.9283 & 0.7026 & 0.4777\\
 MORES $3\times$ IB & 0.3423 & 0.9271 & 0.6980 & 0.4687 \\
 MORES $4\times$ IB & 0.3307 & 0.9322 & 0.6565 & 0.4559\\
%  MORES ClsPool  & 0.3442  & 0.9244 & 0.6721 & 0.4650   \\
%  MORES AvePool  &  0.3415  & 0.9264 & 0.7041 & 0.4729    \\
%  MORES ClsPool Tied  & 0.3456 & 0.9283 & 0.7026 & 0.4777   \\
%  MORES AvePool Tied  & 0.3468 & 0.9671 & 0.7175 & 0.4748   \\
 %\hline
 %FastText+ConvKNRM~\cite{hofstatter2019effect} & 0.2900 & - & - & - & - & - \\
 \hline \hline 
\end{tabular}
\label{tab:perf-marco}
\end{table*}

\begin{table*}[t]
\caption{Average time in seconds to evaluate one query with 1,000 candidate documents.  }

\subcaption{\texttt{MORES} with the Document Representation Reuse Strategy (S1)}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{ c || c c c | c c c }
\hline \hline 
 & \multicolumn{3}{c|}{CPU} & \multicolumn{3}{c}{GPU} \\ 
 Document length $d$ & MORES w/ S1 & BERT ranker & Speedup  & MORES w/ S1 & BERT ranker & Speedup  \\ 
 \hline
  128 & 8.11 & 161.51 & 19.9x & 0.12 & 2.70 & 22.01x\\
 256 & 12.39 & 349.70 & 28.22x & 0.19 & 5.78 & 30.61x\\
 512 &  19.99 & 698.01 & 34.91x & 0.32 & 13.05 & 40.20x\\
 \hline \hline
\end{tabular}}


\subcaption{\texttt{MORES} with the Transformed Document Representation Reuse Strategy (S2) }

\resizebox{0.99\textwidth}{!}{
\begin{tabular}{ c || c c c | c c c }
\hline \hline
 & \multicolumn{3}{c|}{CPU} & \multicolumn{3}{c}{GPU} \\ 
 Document length $d$ & MORES w/ S2 & BERT ranker & Speedup  & MORES w/ S2 & BERT ranker & Speedup  \\ 
 \hline
  128 & 4.52 & 161.51 & 35.7x & 0.05 & 2.70 & 47.94x\\
 256 & 5.18 & 349.70 & 67.55x &  0.07 & 5.78 & 84.71x\\
 512 & 5.63 & 698.00 & 123.89x & 0.10 & 13.05 & 124.08x\\
 \hline \hline 
\end{tabular}}
\label{tab:speed}
\end{table*}
\begin{table*}[t]

\caption{Effectiveness of \texttt{MORES} models and baseline rankers on ClueWeb09-B.}
\centering
\begin{tabular}{ l || c c c || c c c }
\hline \hline
    & \multicolumn{6}{c}{Clueweb09-B} \\ \cline{2-7}
    & \multicolumn{3}{c||}{Title Queries} & \multicolumn{3}{c}{Description Queries} \\ \cline{2-7}
 & NDCG@20 & MAP & Prec@20 & NDCG@20 & MAP & Prec@20  \\  
 \hline
 BERT ranker  & 0.3294  & 0.1882 & 0.3755 & 0.3597 & 0.2075 & 0.3881 \\
 \hline
 MORES $1\times$ IB & 0.3059 & 0.1753 & 0.3407 & 0.3472 & 0.2009 & 0.3705\\
 MORES $2\times$ IB & 0.3317 & 0.1872 & 0.3662 & 0.3571 & 0.2039 & 0.3816\\
 MORES $3\times$ IB & 0.3299 & 0.1841 & 0.3679 & 0.3476 & 0.2008 & 0.3763\\
 MORES $4\times$ IB & 0.3164	& 0.1824 & 0.3515 & 0.3472 & 0.2012 & 0.372\\
 \hline
 adapt-interaction & 0.3179 & 0.1849 & 0.3548 & 0.3385 & 0.1976 & 0.3652\\
 adapt-representation & 0.3319 & 0.1865 & 0.3657 & 0.3557 & 0.2072 & 0.3828\\
 adapt-no-doc & 0.3243 & 0.1862 & 0.3593 & 0.3542 & 0.2054 & 0.3780\\
 \hline \hline 
\end{tabular}
\label{tab:perf-cw}
\end{table*}

\begin{table*}[t]
\caption{Effectiveness of \texttt{MORES} models and baseline rankers on Robust04}
\centering

\begin{tabular}{ l || c c c || c c c }
\hline \hline
    & \multicolumn{6}{c}{Robust04} \\ \cline{2-7}
    & \multicolumn{3}{c||}{Title Queries} & \multicolumn{3}{c}{Description Queries} \\ \cline{2-7}
 & NDCG@20 & MAP & Prec@20 & NDCG@20 & MAP & Prec@20  \\  
 \hline
 BERT ranker  & 0.4632  & 0.2225 & 0.3958 & 0.5065 & 0.245 & 0.4147 \\
 \hline
 MORES $1\times$ IB & 0.4394	& 0.2097 & 0.3741 & 0.4683 & 0.2263 & 0.3835\\
 MORES $2\times$ IB & 0.4599  & 0.2194 & 0.394 & 0.4846 & 0.2323 & 0.4008  \\
 MORES $3\times$ IB & 0.4551	& 0.2135 & 0.3934 & 0.4854 & 0.2334 & 0.4006\\
 MORES $4\times$ IB & 0.4553 & 0.2177 & 0.3938 & 0.4802 & 0.2309 & 0.398 \\
 \hline
 adapt-interaction & 0.4389 & 0.2117 & 0.3723 & 0.4697 & 0.2249 & 0.3896\\
 adapt-representation & 0.4564 & 0.2182 & 0.3926 & 0.4884 & 0.2327 & 0.4042\\
 adapt-no-doc & 0.4429 & 0.2126 & 0.3809 & 0.479 & 0.2282 & 0.3954\\
 \hline \hline 
\end{tabular}
\label{tab:perf-robust}
\end{table*}

This section first study \texttt{MORES}'s ranking effectiveness and efficiency. Then it test the \texttt{MORES} under a domain adaptation setting. An attention analysis is provided to illustrate the behaviors of the Representation and Interaction Modules in \texttt{MORE}. Finally, we study the impacts of the proposed weight initialization method. 

\subsection{Ranking Effectiveness}
\label{sec:marco-ranking}
\autoref{tab:perf-marco} reports the ranking accuracy of \texttt{MORES} and the baseline BERT-based ranker. \zhuyun{mention S1/S2 does not affect accuracy}
 Our experiments show that \texttt{MORES} achieve comparable performance to the BERT ranker on both query sets. %In particular, the MORES AvePool Tied variant achieves no more than 2 percent lower performance compared to the BERT full ranker. It has relatively better performance on some of the evaluations. 

\zhuyun{discuss effects of IB layers!}
On the MS MARCO's Dev Queries,  \texttt{MORES} was able to rank queries with single relevance. On TREC2019 DL Queries, \texttt{MORES} trained over single relevance judgement can generalize to rank candidates for queries with multiple judgments and achieve close to BERT ranker or better performance. 
% \luyu{Remove} Comparing \texttt{MORES} with \texttt{BERT-Siamese} ranker, we found that \texttt{MORES}'s accuracy is significantly higher regardless of model variants. This result proves our hypothesis that global document/query embeddings, although efficient, are not sufficient for accurate ranking. The attention in BERT ranker is critical for modeling interactions between query tokens and document tokens, and it is necessary to retain \emph{token-level} representations as in \texttt{MORES}. 
% Among the four variants, we observe that weight tying can help improve robustness in model training. Average pooling, on the other hand, improve some metrics but also leads to drops in others. 
This collection of results demonstrates that entangled and computationally expensive full-attention transformer can be substituted by \texttt{MORES}'s modularized design with light decoupled query/document attention. \zhuyun{It indicates that it is not necessary to do rep/int simutaniously, Instead, document/query representation can be computed independently without seeing each other. With the contextualized representation, 2 layers of light weighted interaction is sufficient to make a relevance judgment. }
% By storing the token-level representations instead of global query/document embeddings, \texttt{MORES} retains token-level matching information, outperforming the previous representation-based ranking paradigm.  
The \texttt{MORES} framework can achieve competitive ranking performance as the state-of-the-art ranking models.  %but not simple cosine similarity can be used as substitute of self attention in BERT reranker.

\subsection{Ranking Speed}
\luyu{Make this shorter}
The second experiment measures \texttt{MORES}'s real-time processing speed and compared it with measurement for the BERT ranker.   
We record average time for ranking one query with 1000 candidate documents on 8-core CPU and a single GPU. Details can be in \autoref{sec:appendix-eff}. 
We measured ranking speed with document of length 128, 256, 512 with fixed query length of 16. We test both strategies introduced in Section~\ref{sec-reuse} with different time vs. time trade-offs. Table~\ref{tab:speed}(a) and (b) shows the speed tests for the two reuse strategies, correspondingly. 


We observe a substantial speedup in  \texttt{MORES} compared to BERT ranker, and the gain is consistent across CPUs and GPUs. The original BERT ranker took hundreds of seconds -- several minutes -- to generate results for one query on a CPU machine, which is impractical for real-time use. %\texttt{MORES} substantially reduces the ranking time. 
Using the reuse strategy S1, \texttt{MORES} was $20x$ faster than the BERT ranker on shorter documents ($d=128$). The difference is more profound on longer documents. As the length of the document increases, a larger portion of compute in BERT ranker is devoted to performing self-attention over the document sequence. \texttt{MORES} pre-computes document representations and avoids document-side self attention, rending up to $40x$ speedup on longer documents ($d=512$). 

Strategy S2 -- the projected document reuse strategy -- further enlarges the gain in speed, leading to up to $120x$ speedup. Recall that  S2 pre-compute the document projection in \texttt{MORES}'s Interaction Module, which is of $n^2d$ time complexity where $n$ is the model hidden dimension. In practice, $n$ is often large, e.g., our experiment used $n=768$. S2 avoids the expensive $n^2d$ term at evaluation time. 

% As \texttt{MORES} requires data flow from understanding modules to relevance judging module, we expect a higher overhead of \texttt{MORES} than the BERT ranker. The ranking times reported in table \ref{tab:speed} did not exclude those overheads, and we use them as a rough guideline to \texttt{MORES}'s potential. We expect a lower level optimization in C++ will reduce the overheads and further speed up the execution. %we leave that as a future work.

\subsection{Domain Adaptation}
% \zhuyun{explain why people will care about this experiment: .e.g, making earl also available to low resource domains, gain understanding if interaction/representation is more domain specific, etc.}
% \zhuyun{Did we mention experimental settings? e.g., trained on marco, fine-tuned using 5-fold cross validation, etc.} \luyu{TODO: put them in experiment methodologies}
The original BERT reranker can be adapted to low resource domains with a few in-domain examples~\cite{dai2019deeper}. The second experiment study whether \texttt{MORES}'s modularized design affect the transfer ability using Clueweb09-B and Robust. In addition, it test the transfer ability of individual Representation and Interaction modules to gain better understanding. Results are recorded in \autoref{tab:perf-cw} and \autoref{tab:perf-robust}. %We adapt \texttt{MORES} with different interaction round to study their transfer ability. Module adaptation experiments, adapting a \emph{subset} of modules,  also help us better understand behavior of each of \texttt{MORES} modules. 
 
We first examine the effectiveness of adapted the entire \texttt{MORES}.  We observe similar patterns as on MS MARCO: using two to three layers of Interaction Blocks (IB) achieve very close to BERT ranker performance in both datasets for both type of queries, while using a sinlge layer of IB is less effective. Importantly,  our results shows that the modularized design of \texttt{MORES} does not hurt the transfer ability, indicating that new domains and low resource domains can also use \texttt{MORES} through simple adaptation. %Differently, Though perform less effective in MARCO, we found that when using description queries on both dataset, four-time interaction perform very similar to two-time and three-time model, suggesting that it is taking advantage of deeper interaction.

 We observe that only adapting interaction module to the target domain is less effective compared to adapting the entire model, suggesting that changing the behaviours of interaction is not enough to accommodate language changes across domains. On the other hand,  freezing the Interaction Module and only adapting the Representation Modules (adapt-representation) leads performance on par with adapting the entire module. It reveals that the representations need to domain-specific, while the interaction patterns is more general and are not totally dependent on representations. 
% Finally,  freezing document representation module (adapt-no-doc) only slightly lowers the performance compared to a full adaptation, meaning that when receiving new queries, it is possible to update the ranker to query changes without affecting the document index.
%Without changing document representations, this method opens the possibility of 
\subsection{Case Study}
\label{sec:attention-analysis}
Here we demonstrate how to use \texttt{MORES} to understand behaviors in transformer rankers by by visualising the attention weights within the Representation Modules and the Interaction Module.
% The third experiment aims to understand how text is processed within the Representation Modules and the Interaction Module by visualising the attention weights in each module.
%Attention weight is a powerful tool to understand neural models~\cite{mtattention}, especially in \texttt{MORES} where attention operations are assigned dedicated roles of representation (document to document, query to query attention) or interaction (query to document attention). 
%We use a adapted version of BertViz~\cite{bertviz} to demonstrate analysis of \texttt{MORES} attention. As an example, 
% As shown in Figure~\ref{fig: att-vis}, 
We examine a hard to understand query \textit{"what is paranoid sc"} where ``sc" is particularly ambiguous, along with document \textit{"Paranoid schizophrenia is a psychotic disorder...."} As shown in \autoref{fig: att-vis}(a-b),  Representation Modules use attention to contextualize token representations. In the query, due to the short context, ``sc'' incurs a broad but less meaningful attention. On the document side, where the sentence is clear, \textit{"disorder"} use \textit{``psychotic''} and \textit{``schizophrenia''} to contextualize itself.  %and 'we see the token "sc", which a human reader can not easily understand using query only as an not spelled-out "schizophrenia", perplexed the module. 
In \autoref{fig: att-vis}(c-d), we further inspect the two IBs in the Interaction Module. The query token "sc" broadly attention over the document in the first IB to further disambiguate itself, and activate salient attention to "schizophrenia" in the second IB to produce relevance signals. This result explains why \texttt{MORES} $1 \times$ IB performs worse than \texttt{MORES} with more IB layrs -- the ambiguous query needs to gather context from the document before making relevance judgements in the second IB. 
%We acknowledge that the execution suffers from a variety of overheads, especially for MORES running on GPU, such as communication between python interpreter and Pytorch library and python's global interpreter lock. 
    
% \subsection{Light MORES Ranking Effectiveness}

% \begin{table}[!ht]
% \caption{Ranking accuracy of \texttt{MORES} with varying number of judger blocks. The models were tested on the MS MARCO dataset with the Dev Queries.}
% \centering
% \begin{tabular}{ l || c }
% \hline \hline 
% Model & Dev Queries \\
%  & MRR@10 \\
%  \hline
% BERT Ranker & 0.352 \\
% MORES ClsPool & 0.346 \\
% Light MORES & 0.322 \\
%  \hline \hline 
% \end{tabular}
% \label{tab: compress}
% \caption{Effects of introducing Re-contextualizer}
% \end{table}

% To examine the re-contextualization effectiveness, we train an \texttt{Light MORES} model with 2-layer interaction module, using techniques described in section~\ref{subsec: training-techniques}. We evaluate the model on MARCO Dev Queries and record performance and record performance in table~\ref{tab: compress}. Here, we observe that the re-contextualization mechanism, while not able to precisely reach the original representation's expressiveness, is still able to $93\%$ of original model's performance.
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.93\textwidth]{figs/dd_n.pdf}
        \caption{Document Representation}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.93\textwidth]{figs/qq_n.pdf}
        \caption{Query Representation}
    \end{subfigure}
    
%\label{fig: representation-attn}
%\end{figure}
%\begin{figure}[h]
%\centering
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.93\textwidth]{figs/qd_1_n.pdf}
        \caption{Interaction (1st IB)}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.93\textwidth]{figs/qd_2_n.pdf}
        \caption{Interaction (2nd IB)}
    \end{subfigure}

\caption{Visualization of attention in \texttt{MORES}'s different modules.}

%\caption{Interaction Attentions using 2 layers of IB}
\label{fig: att-vis}
\end{figure}
